Packing a Degree Sequence Realization With A Graph

Two simple $n$-vertex graphs $G_{1}$ and $G_{2}$, with respective maximum degrees $\Delta_{1}$ and $\Delta_{2}$, are said to pack if $G_{1}$ is isomorphic to a subgraph of the complement of $G_{2}$. The BEC conjecture by Bollob\'{a}s, Eldridge, and Catlin, states that if $(\Delta_{1}+1)(\Delta_{2}+1)\leq n+1$, then $G_{1}$ and $G_{2}$ pack. The BEC conjecture is true when $\Delta_{1}=2$ and has been confirmed for a few other classes of graphs with various conditions on $\Delta_{1}$, $\Delta_{2}$, or $n$. We show that if \[(\Delta_{1}+1)(\Delta_{2}+1)\leq n+\min\{\Delta_{1},\Delta_{2}\},\] then there exists a simple graph with an identical degree sequence as $G_{1}$ that packs with $G_{2}$. However, except for a few cases, we show that this bound is not sharp. As a consequence of our work, we confirm the BEC conjecture if $G_{1}$ is the vertex disjoint union of a unigraph and a forest $F$ such that either $F$ has at least $\Delta_{2}+1$ components or at most $2\Delta_{2}-1$ edges.

==> main_unigraph_proof.tex <==
We will first need a couple of helpful lemmas that are interesting by themselves.

\begin{lemma}Let $G_{1}$ and $G_{2}$ be graphs that satisfy (\ref{eq:BEC}),  $G_{1}$ is the disjoint union of two unigraphs $F$ and $H$ such that $|H|\leq \min\{\Delta_{1},\Delta_{2}\}+\Delta_{2}-1$, then $G_{1}$ packs with $G_{2}$.
\begin{proof}The only regular connected unigraphs are a complete graphs. So if $F$ is regular, then we may first pack $F$ with $G_{2}$. This leaves $(\Delta_{1},\Delta_{2}$
    
\end{proof}
\end{lemma}


\begin{lemma}\label{lem:largeMatching}Let $G_{1}$ and $G_{2}$ be simple graphs of order $n$ with $\Delta(G_i)=\Delta_i$ for $i=1,2$ such that $G_{1}$ is the vertex disjoint union of a graph $F$ and a graph $M$ such that $\Delta(M)\leq 1$ and  $|M|
\geq 2\Delta_{2}+1$. If $(\Delta_{1}+1)(\Delta_{2}+1)\leq n+1$, then there is a graph $H$ that is the vertex disjoint union of an $F'\in \mathcal{R}(F)$ and a graph $M'\in \mathcal{R}(M)$ such that $G'_{1}\cup G_{2}$ is a packing.
\begin{proof}Since $(\Delta_{1}+1)(\Delta_{2}+1)\leq n+1$, Corollary~\ref{cor:BECdegree} says we can pack $\pi(F)$ with $G_{2}$. Since there are at least $2\Delta_{2}+1$ vertices of $G_{2}$ that are not packed with $\pi(F)$, Theorem~\ref{theorem:BEC-half} says we can pack $\pi(M)$ with the remaining vertices. This gives us our desired packing.
\end{proof}
\end{lemma}

A split graph is a graph that can be partitioned into complete graph and an independent set. The complement is split and every realization of a split graph is a split graph. \cite{}

\begin{lemma}\label{lem:splitPacking}Let $G_{1}$ and $G_{2}$ be simple graphs of order $n$ with $\Delta(G_i)=\Delta_i$ for $i=1,2$ such that $G_{1}$ is the vertex disjoint union of a split graph $F$ and a graph $M$ such that $\Delta(M)\leq 1$. If $(\Delta_{1}+1)(\Delta_{2}+1)\leq n+1$, then there is a graph $H$ that is the vertex disjoint union of an $F'\in \mathcal{R}(F)$ and a graph $M'\in \mathcal{R}(M)$ such that $G'_{1}\cup G_{2}$ is a packing.
\begin{proof}If $G_{1}$ is a split graph, then the theorem follows from Corollary~\ref{cor:BECdegree}. Moreover, if $\Delta(G_{2})\leq 1$, then $G_{2}$ can be packed with $G_{1}$ by Theorem~\ref{theorem:BEC-half}.  Suppose $G_{1}$ is made up of a connected non-empty split graph $F$ and graph $M$ such that $\Delta(F)\geq 2$ and $\Delta(M)\leq 1$. Thus, $n=|F|+|M|$. By Lemma~\ref{lem:largeMatching}, we may assume $|M|\leq 2\Delta_{2}$. Since $n-|M|\geq \Delta_{1}+2$, we know that $F$ is not a complete graph. Therefore, $F$ is not regular since the only regular split graph is a complete graph. If $|M|\leq \min\{\Delta_{1},\Delta_{2}\}+\Delta_{2}-1$, then we first pack $M$ with $G_{2}$. Since $n-|M|\geq (\Delta_{1}+1)(\Delta_{2}+1)-(\min\{\Delta_{1},\Delta_{2}\}+\Delta_{2})$, Theorem~\ref{theorem:BEC-half} says we can pack $F$ with the untouched vertices of $G_{2}$. Thus, we are left with the situation $2\Delta_{2}\geq |M|\geq \min\{\Delta_{1},\Delta_{2}\}+\Delta_{2}$. This implies 
$\min\{\Delta_{1},\Delta_{2}\}\leq \Delta_{2}$. Therefore, $\Delta_{2}\geq \Delta_{1}$. Let $I$ be the largest independent set in $F$ and $W=V(F)-I$. Every vertex in $W$ is adjacent in $F$ to all other vertices in $W$ and at most $\Delta_{1}-|W|+1$ vertices in $I$. This implies $|W|\leq \Delta_{1}-1\leq \Delta_{2}-1$. 
Therefore, $n-|M|-|W|\leq e_{F}(W,I)\leq |W|(\Delta_{1}-|W|+1)$. Grouping the $|W|$ term onto the right hand side and using our bounds on $\Delta_{1}$ and $|W|$ we see that $n-|M|\leq |W|(\Delta_{1}-|W|+2)\leq (\Delta_{1}-1)(\Delta_{2}-1)$. However, this leads us to a contradiction since  $n-|M|\geq (\Delta_{1}+1)(\Delta_{2}+1)-(2\Delta-{2}-1)=\Delta_{2}(\Delta_{1}-1)+\Delta_{1}+2$. This completes the proof of the lemma.
\end{proof}
\end{lemma}

After spending a few minutes studying Theorem~4 in \cite{Tyshkevich2000} one would see that a connected unigraph $H$ is either split graph or has at most $\Delta(H)+3$ vertices. There is only one type of disconnected unigraph, and that is the disjoint vertex union of a star and a matching. By Theorem~\ref{thm:BECmax2} we may assume both $G_{1}$ and $G_{2}$ have maximum degree at least three. Note that $(\Delta_{1}+1)(\Delta_{2}+1)-(\Delta_{1}+3)=\Delta_{2}(\Delta_{1}+1)-2\geq 2\Delta_{2}+1$. Therefore, if $G_{1}$ is not split, then Lemma~\ref{lem:largeMatching} proves our theorem. If $G_{1}$ is split, then Lemma~\ref{lem:splitPacking} proves our theorem.
